Pre-training Distillation for Large Language Models: A Design Space Exploration

Knowledge distillation (KD) aims to transfer knowledge from a large teacher model to a smaller student model. Previous work applying KD in the field of large language models (LLMs) typically focused on the post-training phase, where the student LLM learns directly from instructions and corresponding responses generated by the teacher model. In this paper, we extend KD to the pre-training phase of LLMs, named pre-training distillation (PD). We first conduct a preliminary experiment using GLM-4-9B as the teacher LLM to distill a 1.9B parameter student LLM, validating the effectiveness of PD. Considering the key impact factors of distillation, we systematically explore the design space of pre-training distillation across four aspects: logits processing, loss selection, scaling law, and offline or online logits. We conduct extensive experiments to explore the design space of pre-training distillation and find better configurations and interesting conclusions, such as larger student LLMs generally benefiting more from pre-training distillation, while a larger teacher LLM does not necessarily guarantee better results. We hope our exploration of the design space will inform future practices in pre-training distillation.

==> 04.discussion.tex <==
\section{Discussions}

\begin{table}[]
    \centering
    \small
\begin{adjustbox}{max width=1\linewidth}{
    \begin{tabular}{lrrrr}
    \toprule
    & 1.9B-100B & 1.9B-500B & 3.8B-100B & 3.8B-500B \\
    \midrule
    LLM-LM & $37.7$ & $46.0$ & $42.0$ & $52.0$ \\
    LLM-KD & $38.3$ & $46.7$ & $44.9$ & $54.5$ \\
    \bottomrule
    \end{tabular}
    }
    \end{adjustbox}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

% Scaling到more tokens

% pruning and distilling
% weak-to-strong
